ThermalSplat: Generalizable Pose-Free Gaussian Splatting for Sparse-View Thermal 3D Reconstruction

Thermal infrared imaging is vital for applications like search-and-rescue and autonomous navigation, yet trans- lating it into 3D scene representations remains a critical bottleneck. The low-texture nature and view-dependent emissivity of thermal images cause standard pose estima- tors to fail catastrophically, collapsing standard 3D Gaus- sian Splatting pipelines under sparse-view constraints. Fur- thermore, existing thermal reconstruction methods rely heavily on dense capture and computationally expensive per-scene optimization. Critically, many of these ap- proaches depend on aligned RGB-thermal datasets to ob- tain reliable camera poses and initial point clouds, ren- dering them unusable in purely thermal, unposed envi- ronments. To break this bottleneck, we present Thermal- Splat, the first generalizable, feed-forward Gaussian splat- ting framework that reconstructs 3D scenes directly from sparse thermal images without requiring known camera poses, RGB guidance, or per-scene training. We over- come thermal-specific challenges using a soft census loss for brightness-invariant structural matching and a bound- ary structure loss to explicitly supervise temperature discon- tinuities. Trained on an aggregated multi-source dataset, ThermalSplat synthesizes sharp reconstructions of unseen scenes in a single feed-forward pass. Extensive experi- ments demonstrate that ThermalSplat holds a strict advan- tage over scene-specific thermal splatting methods in the sparse regime. Furthermore, even compared against these baselines operating under their ideal dense capture set- tings, ThermalSplat achieves superior perceptual fidelity. By eliminating the need for computationally expensive per scene optimization, ThermalSplat offers an efficient and generalizable approach to thermal 3D reconstruction.

==> sec/3_dataset_preperation.tex <==
\section{Dataset}
\label{sec:data}

\subsection{Aggregated Thermal Corpus}
No single existing thermal dataset provides sufficient volume and diversity
for training a generalizable reconstruction model from scratch. We therefore
aggregate scenes from five publicly available multi-view thermal datasets:
MVTV~\cite{xu2024leveraging}, ThermalGaussian~\cite{lu2024thermalgaussian}, Thermal3DGS~\cite{chen2026thermal3d},
ThermalMix~\cite{ozer2024exploring}, and ThermoNeRF~\cite{hassan2025thermonerf}. Together these span indoor
objects, outdoor structures, building facades, low-light scenes, and UAV aerial
captures, providing a diverse range of scene types.
 
\subsection{Preprocessing}

Raw thermal images are single-channel grayscale with scene-dependent radiometric ranges, posing two compatibility issues for the RGB-pretrained backbone. First, to bridge the channel mismatch without modifying the network architecture, each single-channel thermal frame is replicated across three channels to satisfy the input requirements of the backbone. Second, since different thermal cameras operate with different radiometric ranges, calibration settings, and sensor characteristics, a scene-level global normalisation is applied to map all image intensities to a consistent range. To suppress the influence of outlier intensities arising from sensor artifacts or isolated hot spots, normalisation is performed using robust percentile bounds computed across all frames in the sequence. Specifically, each pixel intensity $x$ is normalised as:
\begin{equation}
    \hat{x} = \frac{x - p_{\alpha}}{p_{1-\alpha} - p_{\alpha}}
\end{equation}

\noindent where $p_{\alpha}$ and $p_{1-\alpha}$ denote the lower and upper 
percentile values computed globally across the scene, with $\alpha = 0.01$ 
corresponding to the 1st and 99th percentiles~\cite{Gonzalez2008}. Values of $\hat{x}$ are subsequently clipped to $[0, 1]$ to handle the small 
fraction of pixels that fall outside the percentile bounds.
Frame-to-frame radiometric drift, a known characteristic of thermal sensors, is additionally suppressed by removing slow global intensity trends across the sequence prior to scene-level scaling.
 


